Two-Higgs Doublet Model Effective Field Theory

We construct the general two-Higgs doublet model effective field theory where the effects of additional new physics are parameterized by operators up to mass dimension-six. We further transform this effective theory to the Higgs basis and provide matching of the Wilson coefficients between the two descriptions. We illustrate the advantages of the Higgs basis which include the separation of operators that modify standard model couplings and masses from operators that contribute to scattering processes only, transparent correlations between scattering processes resulting from the same operator, and derivation of correlations between different operators in specific UV completions. For completeness, we also construct specific versions corresponding to four types of two-Higgs doublet models: type-I, -II, -X, and -Y, distinguished by $Z_2$ symmetries which restrict the couplings of the Higgs doublets to standard model fermions. Furthermore, we derive general vacuum and stability conditions of the scalar potential in the presence of higher-dimensional terms.

==> main-references.tex <==
%\cite{Appelquist:1974tg}
\bibitem{Appelquist:1974tg}
T.~Appelquist and J.~Carazzone,
%``Infrared Singularities and Massive Fields,''
Phys. Rev. D \textbf{11}, 2856 (1975)
doi:10.1103/PhysRevD.11.2856
%2036 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Grzadkowski:2010es}
\bibitem{Grzadkowski:2010es}
B.~Grzadkowski, M.~Iskrzynski, M.~Misiak and J.~Rosiek,
%``Dimension-Six Terms in the Standard Model Lagrangian,''
JHEP \textbf{10}, 085 (2010)
doi:10.1007/JHEP10(2010)085
[arXiv:1008.4884 [hep-ph]].
%2285 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Murphy:2020rsh}
\bibitem{Murphy:2020rsh}
C.~W.~Murphy,
%``Dimension-8 operators in the Standard Model Effective Field Theory,''
JHEP \textbf{10}, 174 (2020)
doi:10.1007/JHEP10(2020)174
[arXiv:2005.00059 [hep-ph]].
%218 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Gildener:1976ih}
\bibitem{Gildener:1976ih}
E.~Gildener and S.~Weinberg,
%``Symmetry Breaking and Scalar Bosons,''
Phys. Rev. D \textbf{13}, 3333 (1976)
doi:10.1103/PhysRevD.13.3333
%603 citations counted in INSPIRE as of 16 Jul 2024

%\cite{Lavoura:1994fv}
\bibitem{Lavoura:1994fv}
L.~Lavoura and J.~P.~Silva,
%``Fundamental CP violating quantities in a SU(2) x U(1) model with many Higgs doublets,''
Phys. Rev. D \textbf{50}, 4619-4624 (1994)
doi:10.1103/PhysRevD.50.4619
[arXiv:hep-ph/9404276 [hep-ph]].
%203 citations counted in INSPIRE as of 03 Jun 2024

%\cite{Lavoura:1994yu}
\bibitem{Lavoura:1994yu}
L.~Lavoura,
%``Signatures of discrete symmetries in the scalar sector,''
Phys. Rev. D \textbf{50}, 7089-7092 (1994)
doi:10.1103/PhysRevD.50.7089
[arXiv:hep-ph/9405307 [hep-ph]].
%43 citations counted in INSPIRE as of 03 Jun 2024

%\cite{Botella:1994cs}
\bibitem{Botella:1994cs}
F.~J.~Botella and J.~P.~Silva,
%``Jarlskog - like invariants for theories with scalars and fermions,''
Phys. Rev. D \textbf{51}, 3870-3875 (1995)
doi:10.1103/PhysRevD.51.3870
[arXiv:hep-ph/9411288 [hep-ph]].
%256 citations counted in INSPIRE as of 20 Jul 2024

%\cite{Davidson:2005cw}
\bibitem{Davidson:2005cw}
S.~Davidson and H.~E.~Haber,
%``Basis-independent methods for the two-Higgs-doublet model,''
Phys. Rev. D \textbf{72}, 035004 (2005)
[erratum: Phys. Rev. D \textbf{72}, 099902 (2005)]
doi:10.1103/PhysRevD.72.099902
[arXiv:hep-ph/0504050 [hep-ph]].
%477 citations counted in INSPIRE as of 16 Jul 2024

%\cite{Crivellin:2016ihg}
\bibitem{Crivellin:2016ihg}
A.~Crivellin, M.~Ghezzi and M.~Procura,
%``Effective Field Theory with Two Higgs Doublets,''
JHEP \textbf{09}, 160 (2016)
doi:10.1007/JHEP09(2016)160
[arXiv:1608.00975 [hep-ph]].
%32 citations counted in INSPIRE as of 18 Jul 2024

%\cite{Karmakar:2017yek}
\bibitem{Karmakar:2017yek}
S.~Karmakar and S.~Rakshit,
%``Higher dimensional operators in 2HDM,''
JHEP \textbf{10}, 048 (2017)
doi:10.1007/JHEP10(2017)048
[arXiv:1707.00716 [hep-ph]].
%15 citations counted in INSPIRE as of 03 Jun 2024

%\cite{Anisha:2019nzx}
\bibitem{Anisha:2019nzx}
Anisha, S.~Das Bakshi, J.~Chakrabortty and S.~Prakash,
%``Hilbert Series and Plethystics: Paving the path towards 2HDM- and MLRSM-EFT,''
JHEP \textbf{09}, 035 (2019)
doi:10.1007/JHEP09(2019)035
[arXiv:1905.11047 [hep-ph]].
%31 citations counted in INSPIRE as of 15 Jul 2024

%\cite{Feruglio:1992wf}
\bibitem{Feruglio:1992wf}
F.~Feruglio,
%``The Chiral approach to the electroweak interactions,''
Int. J. Mod. Phys. A \textbf{8}, 4937-4972 (1993)
doi:10.1142/S0217751X93001946
[arXiv:hep-ph/9301281 [hep-ph]].
%274 citations counted in INSPIRE as of 12 Jul 2024

%\cite{Contino:2010mh}
\bibitem{Contino:2010mh}
R.~Contino, C.~Grojean, M.~Moretti, F.~Piccinini and R.~Rattazzi,
%``Strong Double Higgs Production at the LHC,''
JHEP \textbf{05}, 089 (2010)
doi:10.1007/JHEP05(2010)089
[arXiv:1002.1011 [hep-ph]].
%310 citations counted in INSPIRE as of 17 Jul 2024

%\cite{Brivio:2017vri}
\bibitem{Brivio:2017vri}
I.~Brivio and M.~Trott,
%``The Standard Model as an Effective Field Theory,''
Phys. Rept. \textbf{793}, 1-98 (2019)
doi:10.1016/j.physrep.2018.11.002
[arXiv:1706.08945 [hep-ph]].
%584 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Buchalla:2023hqk}
\bibitem{Buchalla:2023hqk}
G.~Buchalla, F.~K\"onig, C.~M\"uller-Salditt and F.~Pandler,
%``Two-Higgs-doublet model matched to nonlinear effective theory,''
Phys. Rev. D \textbf{110}, no.1, 016015 (2024)
doi:10.1103/PhysRevD.110.016015
[arXiv:2312.13885 [hep-ph]].
%4 citations counted in INSPIRE as of 18 Jul 2024

%\cite{Gorbahn:2015gxa}
\bibitem{Gorbahn:2015gxa}
M.~Gorbahn, J.~M.~No and V.~Sanz,
%``Benchmarks for Higgs Effective Theory: Extended Higgs Sectors,''
JHEP \textbf{10}, 036 (2015)
doi:10.1007/JHEP10(2015)036
[arXiv:1502.07352 [hep-ph]].
%113 citations counted in INSPIRE as of 26 Jun 2024

%\cite{Belusca-Maito:2016dqe}
\bibitem{Belusca-Maito:2016dqe}
H.~B\'elusca-Ma\"\i{}to, A.~Falkowski, D.~Fontes, J.~C.~Rom\~ao and J.~P.~Silva,
%``Higgs EFT for 2HDM and beyond,''
Eur. Phys. J. C \textbf{77}, no.3, 176 (2017)
doi:10.1140/epjc/s10052-017-4745-5
[arXiv:1611.01112 [hep-ph]].
%54 citations counted in INSPIRE as of 15 Jul 2024

%\cite{DasBakshi:2024krs}
\bibitem{DasBakshi:2024krs}
S.~Das Bakshi, S.~Dawson, D.~Fontes and S.~Homiller,
%``Relevance of one-loop SMEFT matching in the 2HDM,''
Phys. Rev. D \textbf{109}, no.7, 075022 (2024)
doi:10.1103/PhysRevD.109.075022
[arXiv:2401.12279 [hep-ph]].
%3 citations counted in INSPIRE as of 18 Jul 2024

%\cite{Branco:2011iw}
\bibitem{Branco:2011iw}
G.~C.~Branco, P.~M.~Ferreira, L.~Lavoura, M.~N.~Rebelo, M.~Sher and J.~P.~Silva,
%``Theory and phenomenology of two-Higgs-doublet models,''
Phys. Rept. \textbf{516}, 1-102 (2012)
doi:10.1016/j.physrep.2012.02.002
[arXiv:1106.0034 [hep-ph]].
%2858 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Dermisek:2023tgq}
\bibitem{Dermisek:2023tgq}
R.~Dermisek, K.~Hermanek, N.~McGinnis and S.~Yoon,
%``Predictions for muon electric and magnetic dipole moments from h\textrightarrow{}\ensuremath{\mu}+\ensuremath{\mu}- in two-Higgs-doublet models with new leptons,''
Phys. Rev. D \textbf{108}, no.5, 055019 (2023)
doi:10.1103/PhysRevD.108.055019
[arXiv:2306.13212 [hep-ph]].
%7 citations counted in INSPIRE as of 15 Jul 2024

%\cite{Gunion:2002zf}
\bibitem{Gunion:2002zf}
J.~F.~Gunion and H.~E.~Haber,
%``The CP conserving two Higgs doublet model: The Approach to the decoupling limit,''
Phys. Rev. D \textbf{67}, 075019 (2003)
doi:10.1103/PhysRevD.67.075019
[arXiv:hep-ph/0207010 [hep-ph]].
%1019 citations counted in INSPIRE as of 16 Jul 2024

%\cite{Krause:2016oke}
\bibitem{Krause:2016oke}
M.~Krause, R.~Lorenz, M.~Muhlleitner, R.~Santos and H.~Ziesche,
%``Gauge-independent Renormalization of the 2-Higgs-Doublet Model,''
JHEP \textbf{09}, 143 (2016)
doi:10.1007/JHEP09(2016)143
[arXiv:1605.04853 [hep-ph]].
%111 citations counted in INSPIRE as of 18 Jul 2024

%\cite{Bijnens:2018rqw}
\bibitem{Bijnens:2018rqw}
J.~Bijnens, J.~Oredsson and J.~Rathsman,
%``Scalar Kinetic Mixing and the Renormalization Group,''
Phys. Lett. B \textbf{792}, 238-243 (2019)
doi:10.1016/j.physletb.2019.03.051
[arXiv:1810.04483 [hep-ph]].
%9 citations counted in INSPIRE as of 03 Jun 2024

%\cite{Weinberg:1979sa}
\bibitem{Weinberg:1979sa}
S.~Weinberg,
%``Baryon and Lepton Nonconserving Processes,''
Phys. Rev. Lett. \textbf{43}, 1566-1570 (1979)
doi:10.1103/PhysRevLett.43.1566
%2447 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Liao:2010ny}
\bibitem{Liao:2010ny}
Y.~Liao,
%``Neutrino Mass Operators of Dimension up to Nine in Two-Higgs-doublet Model,''
Phys. Lett. B \textbf{698}, 288-292 (2011)
doi:10.1016/j.physletb.2011.03.025
[arXiv:1010.5326 [hep-ph]].
%13 citations counted in INSPIRE as of 03 Jun 2024

%\cite{Dedes:2017zog}
\bibitem{Dedes:2017zog}
A.~Dedes, W.~Materkowska, M.~Paraskevas, J.~Rosiek and K.~Suxho,
%``Feynman rules for the Standard Model Effective Field Theory in R$_{ξ}$ -gauges,''
JHEP \textbf{06}, 143 (2017)
doi:10.1007/JHEP06(2017)143
[arXiv:1704.03888 [hep-ph]].
%135 citations counted in INSPIRE as of 15 Jul 2024

%\cite{Haber:1978jt}
\bibitem{Haber:1978jt}
H.~E.~Haber, G.~L.~Kane and T.~Sterling,
%``The Fermion Mass Scale and Possible Effects of Higgs Bosons on Experimental Observables,''
Nucl. Phys. B \textbf{161}, 493-532 (1979)
doi:10.1016/0550-3213(79)90225-6
%621 citations counted in INSPIRE as of 21 Jun 2024

%\cite{Gunion:1989we}
\bibitem{Gunion:1989we}
J.~F.~Gunion, H.~E.~Haber, G.~L.~Kane and S.~Dawson,
%``The Higgs Hunter's Guide,''
Front. Phys. \textbf{80}, 1-404 (2000)
doi:10.1201/9780429496448
%1282 citations counted in INSPIRE as of 03 Jul 2024

%\cite{Fayet:1974pd}
\bibitem{Fayet:1974pd}
P.~Fayet,
%``Supergauge Invariant Extension of the Higgs Mechanism and a Model for the electron and Its Neutrino,''
Nucl. Phys. B \textbf{90}, 104-124 (1975)
doi:10.1016/0550-3213(75)90636-7
%1271 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Aoki:2008av}
\bibitem{Aoki:2008av}
M.~Aoki, S.~Kanemura and O.~Seto,
%``Neutrino mass, Dark Matter and Baryon Asymmetry via TeV-Scale Physics without Fine-Tuning,''
Phys. Rev. Lett. \textbf{102}, 051805 (2009)
doi:10.1103/PhysRevLett.102.051805
[arXiv:0807.0361 [hep-ph]].
%348 citations counted in INSPIRE as of 28 Jun 2024

%\cite{Goh:2009wg}
\bibitem{Goh:2009wg}
H.~S.~Goh, L.~J.~Hall and P.~Kumar,
%``The Leptonic Higgs as a Messenger of Dark Matter,''
JHEP \textbf{05}, 097 (2009)
doi:10.1088/1126-6708/2009/05/097
[arXiv:0902.0814 [hep-ph]].
%84 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Broggio:2014mna}
\bibitem{Broggio:2014mna}
A.~Broggio, E.~J.~Chun, M.~Passera, K.~M.~Patel and S.~K.~Vempati,
%``Limiting two-Higgs-doublet models,''
JHEP \textbf{11}, 058 (2014)
doi:10.1007/JHEP11(2014)058
[arXiv:1409.3199 [hep-ph]].
%179 citations counted in INSPIRE as of 19 Jul 2024

%\cite{Abe:2015oca}
\bibitem{Abe:2015oca}
T.~Abe, R.~Sato and K.~Yagyu,
%``Lepton-specific two Higgs doublet model as a solution of muon g \ensuremath{-} 2 anomaly,''
JHEP \textbf{07}, 064 (2015)
doi:10.1007/JHEP07(2015)064
[arXiv:1504.07059 [hep-ph]].
%115 citations counted in INSPIRE as of 18 Jul 2024

%\cite{Dermisek:2020cod}
\bibitem{Dermisek:2020cod}
R.~Dermisek, K.~Hermanek, N.~McGinnis and N.~McGinnis,
%``Highly Enhanced Contributions of Heavy Higgs Bosons and New Leptons to Muon $g$\ensuremath{-}2 and Prospects at Future Colliders,''
Phys. Rev. Lett. \textbf{126}, no.19, 191801 (2021)
doi:10.1103/PhysRevLett.126.191801
[arXiv:2011.11812 [hep-ph]].
%33 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Dermisek:2021ajd}
\bibitem{Dermisek:2021ajd}
R.~Dermisek, K.~Hermanek and N.~McGinnis,
%``Muon g-2 in two-Higgs-doublet models with vectorlike leptons,''
Phys. Rev. D \textbf{104}, no.5, 055033 (2021)
doi:10.1103/PhysRevD.104.055033
[arXiv:2103.05645 [hep-ph]].
%50 citations counted in INSPIRE as of 18 Jul 2024

%\cite{Barnett:1983mm}
\bibitem{Barnett:1983mm}
R.~M.~Barnett, G.~Senjanovic, L.~Wolfenstein and D.~Wyler,
%``Implications of a Light Higgs Scalar,''
Phys. Lett. B \textbf{136}, 191-195 (1984)
doi:10.1016/0370-2693(84)91179-1
%68 citations counted in INSPIRE as of 03 Jun 2024

%\cite{Barnett:1984zy}
\bibitem{Barnett:1984zy}
R.~M.~Barnett, G.~Senjanovic and D.~Wyler,
%``Tracking Down Higgs Scalars With Enhanced Couplings,''
Phys. Rev. D \textbf{30}, 1529 (1984)
doi:10.1103/PhysRevD.30.1529
%71 citations counted in INSPIRE as of 03 Jun 2024

%\cite{Martin:1997ns}
\bibitem{Martin:1997ns}
S.~P.~Martin,
%``A Supersymmetry primer,''
Adv. Ser. Direct. High Energy Phys. \textbf{18}, 1-98 (1998)
doi:10.1142/9789812839657\_0001
[arXiv:hep-ph/9709356 [hep-ph]].
%4861 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Dermisek:2023rvv}
\bibitem{Dermisek:2023rvv}
R.~Dermisek, K.~Hermanek, T.~Lee, N.~McGinnis and S.~Yoon,
%``Multi-Higgs boson signals of a modified muon Yukawa coupling at a muon collider,''
Phys. Rev. D \textbf{109}, no.9, 095003 (2024)
doi:10.1103/PhysRevD.109.095003
[arXiv:2311.05078 [hep-ph]].
%6 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Dermisek:2023nhe}
\bibitem{Dermisek:2023nhe}
R.~Dermisek, K.~Hermanek, N.~McGinnis and S.~Yoon,
%``Effective field theory of chirally enhanced muon mass and dipole operators,''
Phys. Rev. D \textbf{107}, no.9, 095043 (2023)
doi:10.1103/PhysRevD.107.095043
[arXiv:2302.14144 [hep-ph]].
%5 citations counted in INSPIRE as of 18 Jul 2024

%\cite{Dermisek:2022aec}
\bibitem{Dermisek:2022aec}
R.~Dermisek, K.~Hermanek, N.~McGinnis and S.~Yoon,
%``Ellipse of Muon Dipole Moments,''
Phys. Rev. Lett. \textbf{129}, no.22, 221801 (2022)
doi:10.1103/PhysRevLett.129.221801
[arXiv:2205.14243 [hep-ph]].
%13 citations counted in INSPIRE as of 22 Jul 2024

%\cite{ATLAS:2024lyh}
\bibitem{ATLAS:2024lyh}
G.~Aad \textit{et al.} [ATLAS],
%``Interpretations of the ATLAS measurements of Higgs boson production and decay rates and differential cross-sections in $pp$ collisions at $\sqrt{s}=13$ TeV,''
[arXiv:2402.05742 [hep-ex]].
%13 citations counted in INSPIRE as of 20 Jul 2024

%\cite{Accettura:2023ked}
\bibitem{Accettura:2023ked}
C.~Accettura, D.~Adams, R.~Agarwal, C.~Ahdida, C.~Aim\`e, N.~Amapane, D.~Amorim, P.~Andreetto, F.~Anulli and R.~Appleby, \textit{et al.}
%``Towards a muon collider,''
Eur. Phys. J. C \textbf{83}, no.9, 864 (2023)
[erratum: Eur. Phys. J. C \textbf{84}, no.1, 36 (2024)]
doi:10.1140/epjc/s10052-023-11889-x
[arXiv:2303.08533 [physics.acc-ph]].
%106 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Maltoni:2001dc}
\bibitem{Maltoni:2001dc}
F.~Maltoni, J.~M.~Niczyporuk and S.~Willenbrock,
%``The Scale of fermion mass generation,''
Phys. Rev. D \textbf{65}, 033004 (2002)
doi:10.1103/PhysRevD.65.033004
[arXiv:hep-ph/0106281 [hep-ph]].
%52 citations counted in INSPIRE as of 11 Jul 2024

%\cite{Allwicher:2021jkr}
\bibitem{Allwicher:2021jkr}
L.~Allwicher, L.~Di Luzio, M.~Fedele, F.~Mescia and M.~Nardecchia,
%``What is the scale of new physics behind the muon g-2?,''
Phys. Rev. D \textbf{104}, no.5, 055035 (2021)
doi:10.1103/PhysRevD.104.055035
[arXiv:2105.13981 [hep-ph]].
%24 citations counted in INSPIRE as of 12 Jul 2024

%\cite{DiLuzio:2016sur}
\bibitem{DiLuzio:2016sur}
L.~Di Luzio, J.~F.~Kamenik and M.~Nardecchia,
%``Implications of perturbative unitarity for scalar di-boson resonance searches at LHC,''
Eur. Phys. J. C \textbf{77}, no.1, 30 (2017)
doi:10.1140/epjc/s10052-017-4594-2
[arXiv:1604.05746 [hep-ph]].
%67 citations counted in INSPIRE as of 17 Jul 2024

%\cite{Remmen:2019cyz}
\bibitem{Remmen:2019cyz}
G.~N.~Remmen and N.~L.~Rodd,
%``Consistency of the Standard Model Effective Field Theory,''
JHEP \textbf{12}, 032 (2019)
doi:10.1007/JHEP12(2019)032
[arXiv:1908.09845 [hep-ph]].
%111 citations counted in INSPIRE as of 18 Jul 2024

%\cite{Remmen:2020uze}
\bibitem{Remmen:2020uze}
G.~N.~Remmen and N.~L.~Rodd,
%``Signs, spin, SMEFT: Sum rules at dimension six,''
Phys. Rev. D \textbf{105}, no.3, 036006 (2022)
doi:10.1103/PhysRevD.105.036006
[arXiv:2010.04723 [hep-ph]].
%44 citations counted in INSPIRE as of 22 Jul 2024

%\cite{Remmen:2022orj}
\bibitem{Remmen:2022orj}
G.~N.~Remmen and N.~L.~Rodd,
%``Spinning sum rules for the dimension-six SMEFT,''
JHEP \textbf{09}, 030 (2022)
doi:10.1007/JHEP09(2022)030
[arXiv:2206.13524 [hep-ph]].
%14 citations counted in INSPIRE as of 19 Jul 2024

%\cite{Jenkins:2013zja}
\bibitem{Jenkins:2013zja}
E.~E.~Jenkins, A.~V.~Manohar and M.~Trott,
%``Renormalization Group Evolution of the Standard Model Dimension Six Operators I: Formalism and lambda Dependence,''
JHEP \textbf{10}, 087 (2013)
doi:10.1007/JHEP10(2013)087
[arXiv:1308.2627 [hep-ph]].
%587 citations counted in INSPIRE as of 17 Jul 2024

%\cite{Jenkins:2013wua}
\bibitem{Jenkins:2013wua}
E.~E.~Jenkins, A.~V.~Manohar and M.~Trott,
%``Renormalization Group Evolution of the Standard Model Dimension Six Operators II: Yukawa Dependence,''
JHEP \textbf{01}, 035 (2014)
doi:10.1007/JHEP01(2014)035
[arXiv:1310.4838 [hep-ph]].
%593 citations counted in INSPIRE as of 16 Jul 2024

%\cite{Alonso:2013hga}
\bibitem{Alonso:2013hga}
R.~Alonso, E.~E.~Jenkins, A.~V.~Manohar and M.~Trott,
%``Renormalization Group Evolution of the Standard Model Dimension Six Operators III: Gauge Coupling Dependence and Phenomenology,''
JHEP \textbf{04}, 159 (2014)
doi:10.1007/JHEP04(2014)159
[arXiv:1312.2014 [hep-ph]].
%768 citations counted in INSPIRE as of 16 Jul 2024

%\cite{Dawson:2020oco}
\bibitem{Dawson:2020oco}
S.~Dawson, S.~Homiller and S.~D.~Lane,
%``Putting standard model EFT fits to work,''
Phys. Rev. D \textbf{102}, no.5, 055012 (2020)
doi:10.1103/PhysRevD.102.055012
[arXiv:2007.01296 [hep-ph]].
%98 citations counted in INSPIRE as of 19 Jul 2024

%\cite{Aebischer:2020lsx}
\bibitem{Aebischer:2020lsx}
J.~Aebischer and J.~Kumar,
%``Flavour violating effects of Yukawa running in SMEFT,''
JHEP \textbf{09}, 187 (2020)
doi:10.1007/JHEP09(2020)187
[arXiv:2005.12283 [hep-ph]].
%22 citations counted in INSPIRE as of 25 Jun 2024

%\cite{Baratella:2020lzz}
\bibitem{Baratella:2020lzz}
P.~Baratella, C.~Fernandez and A.~Pomarol,
%``Renormalization of Higher-Dimensional Operators from On-shell Amplitudes,''
Nucl. Phys. B \textbf{959}, 115155 (2020)
doi:10.1016/j.nuclphysb.2020.115155
[arXiv:2005.07129 [hep-ph]].
%50 citations counted in INSPIRE as of 12 Jul 2024
